Heavy-Hitter Detection Entirely in the Data Plane

Identifying the "heavy hitter" flows or flows with large traffic volumes in the data plane is important for several applications e.g., flow-size aware routing, DoS detection, and traffic engineering. However, measurement in the data plane is constrained by the need for line-rate processing (at 10-100Gb/s) and limited memory in switching hardware. We propose HashPipe, a heavy hitter detection algorithm using emerging programmable data planes. HashPipe implements a pipeline of hash tables which retain counters for heavy flows while evicting lighter flows over time. We prototype HashPipe in P4 and evaluate it with packet traces from an ISP backbone link and a data center. On the ISP trace (which contains over 400,000 flows), we find that HashPipe identifies 95% of the 300 heaviest flows with less than 80KB of memory.

==> analysis.tex <==
%%\section{Analysis}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}

%Discuss heaps/ideal space-saving to be used as reference

%\subsection{All probes available at once}
%\subsubsection{Aggregate Model}
%\subsubsection{Cash Register Model}
%\subsection{Accomodating HW constraints}
%\subsubsection{Aggregate Model}
%\subsubsection{Cash Register Model}

%% \subsection{Algorithm}

%% Let table $T$ represent a table of items and corresponding counts. The table has
%% a fixed size $M$, with some table locations possibly empty. A nonempty table
%% location contains an element $e$ and a corresponding counter $c$, denoted as
%% $(e,c)$. Each incoming item $p$, \eg a packet, is independently hashed to $d$
%% locations in table $T$, denoted by the set $H_p$. Consider the following
%% algorithm.\\

%% \noindent For each item $p$\\
%% hash $p$ to table locations $H_p = \{l_1, l_2, \ldots, l_d\}$ with $l_i = (e_i, c_i)$\\
%% if $\exists i: p = e_i$ then $c_i \leftarrow c_i + 1$\\
%% else if $\exists j: l_j$ empty then $e_j \leftarrow p; c_j \leftarrow 1$\\
%% else let $k \leftarrow \mathrm{arg min}_{k \in \{1,\ldots,d\}} \ c_k; e_k \leftarrow p; c_k \leftarrow c_k + 1$\\

\section{Overestimation Errors}
\label{sec:analysis}

We show that \Baseline (\Alg{Baseline}) does not overestimate keys by too much
when it samples the minimum of $d$ slots in the table, instead of the entire
table.

First, note how it is possible to overestimate the frequency of an item
$e_i$. Suppose on its insertion $e_i$ replaces another item $e_j$ in $T$, where
$e_j$ is the element with the minimum counter among locations that $e_i$ hashed
to. Independent of the true count of item $e_i$ so far (say, zero), its counter
is set to $c_j + 1$.

\begin{lemma}
For any item $e_i$ in $T$ (with table count $c_i$), let $min_i$ denote the
minimum counter value among the locations that $e_i$ hashes to. That is, $min_i
= \mathrm{min}_{(e_j,c_j) \in H_i} \ c_j$. Let $f_i$ denote the true count of
$e_i$. Then, $c_i \leq f_i + min_i$.
\end{lemma}

\begin{proof}
Consider an item $e_i$ in $T$, and the last time that $e_i$ was inserted into
the table. Suppose the minimum counter value among the $d$ locations that $e_i$
hashed to at the time of its insertion be $m_i$. Also suppose that $e_i$
occurred $n_i$ times after its last insertion in the table. Clearly, $c_i = m_i
+ n_i$.

The minimum counter among the $d$ locations in $H_i$ is monotonically
increasing, since the algorithm never decrements any counters. Hence, $m_i \leq
min_i$. Further, since $n_i$ can be at most $f_i$, the lemma follows.
\end{proof}

\begin{lemma}
For a fixed $\delta \leq 1$, with probability at least $1 - \delta^d$, we have
$min_i < N/\delta M$.
\end{lemma}

\begin{proof}

We wish to bound the value of $min_i$ from above. Suppose there are $N$ packet
arrivals overall. Since every item arrival contributes to an increment in $T$,
the expected value of a counter in $T$ is $N/M.$ Hence, the minimum counter in
$T$ can be at most the expected value, \ie $N/M.$ However, the minimum in $H_i$ for an
item $i$ can in general be quite far from the minimum of $T$.

It can be shown that the minimum in $H_i$ is still unlikely to be much larger
than the bound on the minimum above. The expected value of the counters in $T$
is $N/M$, so by the Markov inequality the probability that a randomly chosen
item has a counter value higher than $N/\delta M$ is no more than
$\delta$. Then, the chance that the minimum of $d$ randomly chosen elements is
higher than $N/\delta M$ is at most $\delta^d$. Hence with probability at least
$1 - \delta^d$, we have $min_i \leq N/\delta M$.

\end{proof}

% \subsection{Underestimation errors}

% It is possible to underestimate the counts of items within the table, or miss
% heavy items entirely, through this algorithm. To see why, consider a simple
% example with $d=2$. Suppose item $e_i$ hashes to two locations $l_1$ and $l_2$,
% occupying location $l_1$ with counter $c_1$. Further, suppose that $l_2$ is
% occupied with another item with count $c_2^{evict} < c_1$. Now an item $e_j$ may
% enter $T$, hashing to locations $l_1$ and $l_3$, where the corresponding counter
% value $c_3 > c_1$. Then $e_j$ will evict $e_i$. However, if $e_i$ returns, the
% counter at $l_2$ may still have a smaller value than the original count of
% $e_i$, \ie $c_2^{reappear} < c_1$. Then the current estimate of item $i$ would
% be smaller than its true count by $c_1 - c_2^{reappear}$. If $c_2^{reappear}$ is
% small enough that $e_i$ is evicted later, and $e_i$ never reappears, the
% algorithm may also miss $e_i$ entirely from the table.

% \noindent {\bf Speculative proof ideas.} We want to show that the impact of
% underestimations on counter values in $T$ is not significant. Suppose we call
% $c_1 - c_2^{reappear}$ the {\em underestimation error.} One specific idea is to
% show that the {\em average-case} underestimation error for items in $T$ is
% small, as follows.

% For the underestimation error to be positive-valued, it is necessary that there
% is an item $e_j$ hashing to $d$ locations---including the location that $e_i$
% resides in---with $d-1$ counter values each larger than $c_1$. When $c_1$ is
% large, the likelihood of $d-1$ randomly chosen counters each being larger than
% $c_1$ must be small. On the other hand, if $c_1$ is small, the underestimation
% error is itself small because the gap between $c_1$ and $c_2^{reappear}$ is
% likely to be small. Putting these two cases together, we hope to show that the
% average-case underestimation error for any item must be small.

want to say that underestimatin is no more than constant times N/M, how many times it gets evicted and everytime it gets evicted what the underestimate amount


